Regularity estimate and sparse approximation of pathwise robust Duncan-Mortensen-Zakai equation

In this paper, we establish an \textit{a priori} estimate for arbitrary-order derivatives of the solution to the pathwise robust Duncan-Mortensen-Zakai (DMZ) equation within the framework of weighted Sobolev spaces. The weight function, which vanishes on the physical boundary, is crucial for the \textit{a priori} estimate, but introduces a loss of regularity near the boundary. Therefore, we employ the Sobolev inequalities and their weighted analogues to sharpen the regularity bound, providing improvements in both classical Sobolev spaces and H{\"o}lder continuity estimates. The refined regularity estimate reinforces the plausibility of the quantized tensor train (QTT) method in [S. Li, Z. Wang, S. S.-T. Yau, and Z. Zhang, IEEE Trans. Automat. Control, 68 (2023), pp. 4405--4412] and provides convergence guarantees of the method. To further enhance the capacity of the method to solve the nonlinear filtering problem in a real-time manner, we reduce the complexity of the method under the assumption of a functional polyadic state drift $f$ and observation $h$. Finally, we perform numerical simulations to reaffirm our theory. For high-dimensional cubic sensor problems, our method demonstrates superior efficiency and accuracy in comparison to the particle filter (PF) and the extended Kalman filter (EKF). Beyond this, for multi-mode problems, while the PF exhibits a lack of precision due to its stochastic nature and the EKF is constrained by its Gaussian assumption, the enhanced method provides an accurate reconstruction of the multi-mode conditional density function.

==> _arxiv_TT_NLF_Regularity/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithm}
\usepackage{algpseudocode}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}
\newsiamremark{fact}{Fact}
\crefname{fact}{Fact}{Facts}

% Sets running headers as well as PDF title and authors
\headers{High order regularity and Sparse approximation of DMZ}{Y. Meng, Z. Wang, S. S-T. Yau and Z. Zhang}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Regularity estimate and sparse approximation of pathwise robust Duncan-Mortensen-Zakai equation \thanks{Submitted to the editors DATE.
\funding{The work of Zhongjian Wang is supported in part by the NTU SUG-023162-00001, MOE AcRF Tier 1 Grant RG17/24.  The work of Stephen S.-T. Yau is supported in part by the National Natural Science Foundation of China (No. 42450242), and the Tsinghua University Education Foundation. The work of Zhiwen Zhang is supported in part by the National Natural Science Foundation of China (No. 92470103 and No. 12171406), Hong Kong RGC grant projects (No. 17304324 and No. 17300325), and Seed Funding for Strategic Interdisciplinary Research Scheme 2021/22 (HKU).}
}}

% Authors: full names plus addresses.
\author{Yuhua Meng\thanks{Department of Mathematics, The University of Hong Kong, Pokfulam Road, Hong Kong SAR, P.R.China.(\email{yvette00@connect.hku.hk.} ) } 
\and Zhongjian Wang\thanks{Division of Mathematical Sciences, School of Physical and Mathematical Sciences, Nanyang
Technological University, 21 Nanyang Link Singapore 637371. \email{zhongjian.wang@ntu.edu.sg.} }
\and Stephen S.T. Yau\thanks{Hetao Institute of Mathematics and Interdisciplinary Sciences (HIMIS), Shenzhen 518000, Guangdong, P. R. China, Beijing Institute of Mathematical Sciences and Applications (BIMSA), Beijing 101408, P. R. China, Department of Mathematical Sciences, Tsinghua University, Beijing 100084, P. R. China
\email{yau@uic.edu.} }
\and Zhiwen Zhang\thanks{Corresponding author. Department of Mathematics, The University of Hong Kong, Pokfulam Road, Hong Kong SAR, P.R.China. Materials Innovation Institute for Life Sciences and Energy (MILES), HKU-SIRI,
Shenzhen, P.R. China. (\email{zhangzw@hku.hk.})}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithm}
\usepackage{algpseudocode}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}
\newsiamremark{fact}{Fact}
\crefname{fact}{Fact}{Facts}

% Sets running headers as well as PDF title and authors
\headers{High order regularity and Sparse approximation of DMZ}{Y. Meng, Z. Wang, S. S-T. Yau and Z. Zhang}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Regularity estimate and sparse approximation of pathwise robust Duncan-Mortensen-Zakai equation \thanks{Submitted to the editors DATE.
\funding{The work of Zhongjian Wang is supported in part by the NTU SUG-023162-00001, MOE AcRF Tier 1 Grant RG17/24.  The work of Stephen S.-T. Yau is supported in part by the National Natural Science Foundation of China (No. 42450242), and the Tsinghua University Education Foundation. The work of Zhiwen Zhang is supported in part by the National Natural Science Foundation of China (No. 92470103 and No. 12171406), Hong Kong RGC grant projects (No. 17304324 and No. 17300325), and Seed Funding for Strategic Interdisciplinary Research Scheme 2021/22 (HKU).}
}}

% Authors: full names plus addresses.
\author{Yuhua Meng\thanks{Department of Mathematics, The University of Hong Kong, Pokfulam Road, Hong Kong SAR, P.R.China.(\email{yvette00@connect.hku.hk.} ) } 
\and Zhongjian Wang\thanks{Division of Mathematical Sciences, School of Physical and Mathematical Sciences, Nanyang
Technological University, 21 Nanyang Link Singapore 637371. \email{zhongjian.wang@ntu.edu.sg.} }
\and Stephen S.T. Yau\thanks{Hetao Institute of Mathematics and Interdisciplinary Sciences (HIMIS), Shenzhen 518000, Guangdong, P. R. China, Beijing Institute of Mathematical Sciences and Applications (BIMSA), Beijing 101408, P. R. China, Department of Mathematical Sciences, Tsinghua University, Beijing 100084, P. R. China
\email{yau@uic.edu.} }
\and Zhiwen Zhang\thanks{Corresponding author. Department of Mathematics, The University of Hong Kong, Pokfulam Road, Hong Kong SAR, P.R.China. Materials Innovation Institute for Life Sciences and Energy (MILES), HKU-SIRI,
Shenzhen, P.R. China. (\email{zhangzw@hku.hk.})}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

